Fine-grained Contrastive Learning for Relation Extraction

Recent relation extraction (RE) works have shown encouraging improvements by conducting contrastive learning on silver labels generated by distant supervision before fine-tuning on gold labels. Existing methods typically assume all these silver labels are accurate and treat them equally; however, distant supervision is inevitably noisy -- some silver labels are more reliable than others. In this paper, we propose fine-grained contrastive learning (FineCL) for RE, which leverages fine-grained information about which silver labels are and are not noisy to improve the quality of learned relationship representations for RE. We first assess the quality of silver labels via a simple and automatic approach we call "learning order denoising," where we train a language model to learn these relations and record the order of learned training instances. We show that learning order largely corresponds to label accuracy -- early-learned silver labels have, on average, more accurate labels than later-learned silver labels. Then, during pre-training, we increase the weights of accurate labels within a novel contrastive learning objective. Experiments on several RE benchmarks show that FineCL makes consistent and significant performance gains over state-of-the-art methods.

==> _9_ethics.tex <==
\section{Ethical Concerns}
We do not anticipate any major ethical concerns; relation extraction is a fundamental problem in natural language processing. A minor consideration is the potential for certain types of hidden biases to be introduced into our results (i.e.,~performance regressions for some subset of the data in spite of overall performance gains). We did not observe any such issues in our experiments, and indeed these considerations seem low-risk for the specific datasets studied here because they are all published. 

==> archive/_3_learning_order_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Learning Order Denoising
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Learning order denoising}\label{sec:learning_order}

For learning order denoising, we automatically label large amounts of training data via distant supervision for RE \cite{Mintz2009DistantSF} which we use to train a PLM to predict relation classes using multi-class cross-entropy loss. 
\begin{equation}\label{eq:cross_entropy}
\begin{aligned}
\mathcal{L}_{\mathrm{CE}}=-\sum_{i=1}^{N} y_{o,i} \cdot \log \left(p\left(y_{o,i}\right)\right)
\end{aligned}
\end{equation}
Where the number of classes $N$ is the number of relation classes plus one for \textit{no relation}, $y$ is a binary indicator that is 1 \textit{iff} $i$ is the correct classification for observation $o$, and $p(y_{o,i})$ is the Softmax probability that observation $o$ is of class $i$.

During training, we record the order of training instances learned. An instance is considered ``learned'' upon the initial correct prediction. Likewise, an instance is ``not learned'' if the model fails to correctly predict it before training completes. Training instances are evaluated by batch within each epoch, exposing the model to all training data points the same number of times.

Thus, the PLM is effectively utilized as a mapping function that maps all training instances ($\mathcal{T}$) into two subsets: learned ($\mathcal{A}$) and not learned instances ($\mathcal{B}$) such that $\mathcal{A} \bigcup \mathcal{B}  = \mathcal{T}^\prime$ and $ \mathcal{A} \bigcap \mathcal{B} = \emptyset$.

The set of learned instances $\mathcal{A}$ is further divided into non-intersecting subsets of learned instances $\mathcal{A}_{1}$ through $\mathcal{A}_{k}$ where $k$ corresponds to the epoch in which an instance is learned.
\begin{gather}
\mathcal{A}_{0} \bigcup \mathcal{A}_{1} ... \bigcup \mathcal{A}_{k} = \mathcal{A}\\
\mathcal{A}_{i} \bigcap \mathcal{A}_{j}=\emptyset \text { for all } i \neq j
\end{gather}
We use $k=15$ epochs, resulting in $k+1$ subsets of instances---$k$ subsets of learned instances plus one subset of not learned instances. Figure \ref{fig:ratio_learned} shows the percent of total training instances learned per epoch during this phase on the DocRED distantly labeled training set.

%  Ratio of data learned during learning order phase
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/ratio_learned_bars.pdf}
    \caption{Percent of total training instances learned per epoch when recording learning order during Stage 1 of \our on the DocRED distantly labeled training set.}
    \label{fig:ratio_learned}
\end{figure}

More challenging relation classes may be underrepresented within the set of learned instances. Such minority classes can be problematic during pre-training since unlearned instances are weighted less than learned ones, presenting a challenge for the model to learn informative representations for minority classes. To account for this, we ensure that at least $P\%$ of instances of each relation class is contained within the set of learned instances. During training, we set $P=50\%$ and observed that 2\% of relation classes are underrepresented within the set of learned instances. We upsample underrepresented classes by randomly selecting unlearned instances from the corresponding class, placing them into one of the $k$ subsets of learned instances $\mathcal{A}$. See Figure \ref{fig:complete_learning_order} in the Appendix for a detailed chart showing the ratio of learned instances by relation class in each epoch. 

Learning order metadata is then inserted into the original training data $\mathcal{T}$, creating a modified training set $\mathcal{T}^\prime$ used for the contrastive learning pre-training stage. 

% 
% Learning order as noise level hypothesis
% 
\subsection{Learning order as noise level hypothesis}\label{sec:learning_order_hypothesis}

We seek to confirm our hypothesis that learning order automatically orders distantly supervised data from clean, high-quality instances to noisy, low-quality instances. However, given the large amount of pre-training data, statistically significant confirmation via manual annotation becomes prohibitively expensive. So, we devise the following experiment to test our hypothesis in lieu of a large manual annotation effort.

We begin with the assumption that a model trained on a dataset without noise will perform better than a model trained on a dataset with noise. Suppose learning order denoising successfully orders instances relative to their noise. In that case, we should observe a boost in performance by training on a subset of early-learned instances compared to a model trained on the complete, noisy dataset.

As reported by \cite{Gao2021ManualEM}, up to 53\% of relation instances labeled via distant supervision are incorrect. Using this estimation, we attempt to use learning order denoising to remove the roughly 50\% of instances that are noisy instances from the DocRED's distantly supervised training set. To do this, we first obtain the learning order of relation instances using the methodology described in Section \ref{sec:learning_order}. Without loss of generalization, we choose RoBERTa \cite{Liu2019RoBERTaAR}, specifically the \textit{roberta-base} checkpoint\footnote{\url{https://huggingface.co/roberta-base}}, as the base model to develop the order of learned instances. 


% Trimmed dataset RE
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l c c c } 
\toprule
    \textbf{Learning order}  & \textbf{Training set} & \textbf{Training set size} & \textbf{F1} \\ \midrule
    \rule{-3pt}{3ex}
        None                    & $\mathcal{T}$                             & 100\%      & 45.8 \\
    \rule{-3pt}{3ex}
        Batch-based             & $\mathcal{T}^{\prime}_{\mathcal{A}_0^B}$  & 45.0\%     & \textbf{46.6}\\
    \rule{-3pt}{3ex}
        Epoch-based             & $\mathcal{T}^{\prime}_{\mathcal{A}_0^E}$  & 64.9\%     & 46.0 \\
\bottomrule
\end{tabular}} %end resize
\caption{Results comparing performance on the DocRED test set using trimmed sets of distantly supervised training data. The batch-based and epoch-based training sets consist of training instances determined by the instances learned in the first epoch using the respective learning order collection methods.}
\label{tab:batch_vs_epoch_based}
\end{table}

We observe that the set of training instances learned per batch in the first epoch, $\mathcal{A}_0$, consists of 45\% of the total training instances. We use $\mathcal{A}_0$ to construct a trimmed ``batch-based'' training set $\mathcal{T}^{\prime}_{\mathcal{A}_0}$. We then compare performance in two different settings: (1) RoBERTa trained with the complete distantly supervised training dataset $\mathcal{T}$ and (2) RoBERTa trained on the trimmed, denoised ``batch-based'' training data $\mathcal{T}^{\prime}_{\mathcal{A}_0^B}$. Table \ref{tab:batch_vs_epoch_based} reports the results of this experiment. Significantly, the denoised training set consisting of only 45\% of the complete training data outperforms the baseline model. We use these results to argue that learning order successfully orders instances from clean, high-quality to noisy, low-quality instances. 

We also conduct an informal manual analysis of the learning order. We randomly selected 120 instances from the first six training epochs---60 correctly predicted and 60 incorrectly predicted instances. We find that 93\% of the correct predictions have accurate labels within the first three epochs. However, in epochs 4 through 6, label accuracy drops to 53\% among correct predictions. Furthermore, we find a relatively low label accuracy of 50\% from the first three epochs of incorrect predictions, illustrating that the model struggles to learn noisy instances compared to clean instances early in training. 
%These results and the positive results from experiments in subsequent sections offer additional evidence that earlier learned instances are, on average, cleaner than those learned later in training.


% 
% Batch-based vs Epoch-based
% 
\subsection{Learning order: batch- vs. epoch-based}
We collect learned instances per batch during training and bin them by the epoch in which they were learned. However, we recognize that this may bias the set of learned instances by the batch they are randomly selected for. For example, accurately labeled relation instances selected for the first few batches during training may not be predicted correctly because the model has not learned much. To reduce this bias, we conduct an experiment where we collect learned instances by evaluating the model on the entire training set at the end of each epoch. We name this version ``epoch-based'' learning order. We rerun the experiment detailed in Section \ref{sec:learning_order_hypothesis} using epoch-based learning order to construct the trimmed dataset $\mathcal{T}^{\prime}_{\mathcal{A}_0^E}$ and present the results in Table \ref{tab:batch_vs_epoch_based}.

Using epoch-based learning order, we observe that the model learns 64.9\% of the training instances within the first epoch, an increase compared to the 45.0\% of learned instances from batch-based learning order. However, training RoBERTa on the epoch-based training subset, we obtain an F1 score of 46.0, which under-performs relative to the 46.6 F1 score from the batch-based learning order experiment. We hypothesize that, while epoch-based learning order may capture more learned instances, it leads to noisier instances leaking into the sets of learned data because the model is more prone to simply memorizing noisy labels encountered previously in the epoch. 

Note, we do not use DocRED's human annotated training data in these learning order experiments. Instead, we train on the distantly supervised training data and test on human annotated data. This is done to assess the quality of the various subsets of distantly labeled datasets. It is why the performance of these tests is considerably lower than the results from the experiments in Section \ref{subsec:experiments_relation_extraction} that leverage human annotated training data.




==> archive/_4_finecl_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% FGCL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Contrastive Pre-training}\label{sec:experiments}
%\jingbo{Since we are not following the conventional flow to have method and exp totally separated in different sections, we'd better have an overview paragraph here. Convert all the content before 4.1 into a subsection, focusing on how \our works (probably merge all the method content in this section). We can create smallsections following \textbackslach{}noindent\textbackslach{}textbf\{\#1.\} to give ``subsubsection'' names. For later subsections, make it clear that they are experimental results. The same way of using smallsections apply to dataset, experimental setting discussions. }


% This section introduces our pre-training method to learn high-quality entity and relation representations. Specifically, we use the same method (see Appendix~\ref{app:entity_relation_repr}) as ERICA~\cite{Qin2021ERICAIE} to obtain entity and relation representation for fair comparison. Then, following ERICA, we adopt masked language modeling task (MLM)~\cite{Devlin2019BERTPO} and entity discrimination task (see Appendix~\ref{app:entity}) to avoid catastrophic forgetting~\cite{McCloskey1989CatastrophicII} of general language understanding ability and learn entity representation respectively.

% \bill{This is a suggested re-organization of the paragraph above. We have extra space so I thought it could help to include the additional details of the representation construction. I'm of course open to other ideas if there's a better way to communicate this info.}
This section introduces our pre-training method to learn high-quality entity and relation representations. 

We construct entity and relationship representations following ERICA~\cite{Qin2021ERICAIE}; namely, multiple entities within a document are pooled together via mean pooling to obtain a single representation $\mathbf{e_{j1}}$ per entity. Then, relationship representations are formed by concatenating entity representations of an entity pair: $\mathbf{r}_{j1j2} = [\mathbf{e}_{j1};\mathbf{e}_{j2}]$ (see Appendix~\ref{app:entity_relation_repr} for more details).  

Using these representations, we implement a three-part pre-training objective: entity discrimination, masked language modeling (MLM), and relation discrimination. For entity discrimination, we use the same method described in ERICA (see Appendix~\ref{app:entity_relation_repr}). We include the MLM task~\cite{Devlin2019BERTPO} to avoid catastrophic forgetting of general language understanding~\cite{McCloskey1989CatastrophicII}. Lastly, we design a novel fine-grained relation discrimination objective which is described in detail in the following section. 


\subsection{Fine-grained Contrastive Learning}
%We propose fine-grained contrastive learning for relation representation learning in which the learning order recorded in Section~\ref{sec:learning_order} is used to measure the confidence of different relation instances. For \our, we use the distantly supervised training data augmented with learning order metadata $\mathcal{T}^\prime$ to pre-train RoBERTa. 

%\jingbo{will people be confused between RE and RD? Maybe spend one sentence to explain their relationship and why we are doing RD here.}
To effectively learn representation for downstream task relation extraction, we conduct a Relation Discrimination (RD) task during pre-training.
The goal of RD is to distinguish whether two relations are close or not semantically~\cite{Qin2021ERICAIE}. Existing methods~\cite{Peng2020LearningFC, Qin2021ERICAIE} require large amounts of automatically labeled data from distant supervision (e.g.,~knowledge bases), which is noisy because two sentences with the same entity pair may express different relations (see examples in Section~\ref{sec:introduction}). 

In this case, the learning order can be introduced to let the model be aware of the noise level of relation instances. To efficiently incorporate learning order into the training process, we propose Fine-grained Contrastive Learning (\our) to conduct RD for relation extraction.
%\jingbo{I think the title, abstract, intro are all saying \our is proposed for RE}
In this new method, the noise level of all distantly supervised training instances controls the optimization process by re-weighting the contrastive objective. Intuitively, the model should learn more from high-quality training instances than noisy instances. Hence, we assign higher weights to earlier learned instances from the learning order denoising stage.

In practice, we sample a tuple pair of relation instance $t_A = (d_A, e_{A_1}, r_A, e_{A_2}, k_A)$ and $t_B = (d_B, e_{B_1}, r_B, e_{B_2}, k_B)$ from $\mathcal{T}^\prime$ and $r_A = r_B$, where $d$ is a document; $e$ is a entity in $d$; $r$ is the relationship between two entities and $k$ is the first learned order introduced in Section~\ref{sec:learning_order}. Using the method mentioned in Appendix~\ref{app:entity_relation_repr}, we obtain the positive relation representations $\mathbf{r}_{t_A}$ and $\mathbf{r}_{t_B}$. To discriminate positive examples from negative ones, the fine-grained contrastive loss is defined as follows:
 
\begin{equation}
\begin{aligned}
\mathcal{L}_{\mathrm{RD}} &=-\sum_{t_{A}, t_{B} \in \mathcal{T}^\prime}f(k_A)\log \frac{\exp \left(\cos \left(\mathbf{r}_{t_{A}}, \mathbf{r}_{t_{B}}\right) / \tau\right)}{\mathcal{Z}}, \\
\mathcal{Z} &=\sum_{t_{C} \in \mathcal{T}^\prime /\left\{t_{A}\right\}}^{N} f(k_C)\exp \left(\cos \left(\mathbf{r}_{t_{A}}, \mathbf{r}_{t_{C}}\right) / \tau\right), \\
\end{aligned}
\end{equation}
where $\mathrm{cos}(\cdot,\cdot)$ denotes the cosine similarity; $\tau$ is the temperature; $N$ is a hyper-parameter and $t_{C}$ is a negative instance ($r_A \neq r_C$) sampled from $\mathcal{T}^\prime$. Relation instances $t_A$ and $t_C$ are re-weighted by function $f$ which is defined as:
\begin{equation}
    f(k) = \alpha^{\frac{k_{\mathrm{max}}-k}{k_{\mathrm{max}}- k_{\mathrm{min}}}},
\end{equation}
where $\alpha$ ($\alpha > 1$) is a hyper-parameter that weighs the negative samples; $\mathrm{max}$ and $\mathrm{min}$ are maximum and minimum first-learned order respectively. We increase the weight of negative $t_C$ if it is a high-quality training instance (i.e.,~$k$ is small). Because all positives and negatives are discriminated from instance $t_A$, we control the overall weight by the learning order $k_A$.

% \mathcal{L}_{\mathrm{RD}} &=\mathcal{L}_{\mathrm{RD}}^{\mathcal{T}_{s}^{+}, \mathcal{T}_{s}^{+}}+\mathcal{L}_{\mathrm{RD}}^{\mathcal{T}_{s}^{+}, \mathcal{T}_{c}^{+}}+\mathcal{L}_{\mathrm{RD}}^{\mathcal{T}_{c}^{+}, \mathcal{T}_{s}^{+}}+\mathcal{L}_{\mathrm{RD}}^{\mathcal{T}_{c}^{+}, \mathcal{T}_{c}^{+}}
% \end{aligned}
The overall learning objective of Stage 2 is formulated as follows:
\begin{equation}
\mathcal{L} = \mathcal{L}_{ED} + \mathcal{L}_{RD} + \mathcal{L}_{MLM} 
\end{equation}
where $\mathcal{L}_{MLM}$ and $\mathcal{L}_{ED}$ are objectives of masked language modeling and entity discrimination (Appendix~\ref{app:entity}), respectively. $\mathcal{L}_{RD}$ is our proposed fine-grained contrastive loss. 

% 
% Pre-training
% 
\subsection{Pre-training Details}
To ensure a fair comparison and highlight the effectiveness of Fine-grained Contrastive Learning, we align our pre-training data and settings to those used by ERICA. The pre-training dataset provided by \cite{Qin2021ERICAIE} is constructed using distant supervision for RE by pairing documents from Wikipedia (English) with the Wikidata knowledge graph. This distantly labeled dataset creation method mirrors the method used to create the distantly labeled training set in DocRED \cite{docred} but differs in that it is much larger and more diverse. It contains 1M documents, 7.2M relation instances, and 1040 relation types compared to DocRED's 100k documents, 1.5M relation instances, and 96 relation types (not including \textit{no relation}). Additional checks are performed to ensure no fact triples overlap between the training data and the test sets of the various downstream RE tasks.


% 
% Relation Extraction
% 
\subsection{Relation Extraction}\label{subsec:experiments_relation_extraction}
The primary focus of our work is to improve relationship representations learned during pre-training and, in doing so, improve performance on downstream RE tasks. To illustrate the effectiveness of our pre-training method, we use cross-entropy loss, as described in equation \ref{eq:cross_entropy}, to fine-tune our pre-trained \our model on document-level and sentence-level RE tasks. The baselines are pre-trained and fine-tuned with identical data and settings for a fair comparison.

\textbf{Document-level RE}: To assess our framework's ability to extract document-level relations, we report performance on DocRED \cite{docred}. We compare our model to the following baselines: (1) CNN \cite{zeng-etal-2014-relation}, (2) BiLSTM \cite{lstm}, (3) BERT \cite{Devlin2019BERTPO}, (4) RoBERTa \cite{Liu2019RoBERTaAR}, (5) MTB \cite{BaldiniSoares2019MatchingTB}, (6) CP \cite{Peng2020LearningFC}, (7 \& 8) ERICA\textsubscript{BERT} \& ERICA\textsubscript{RoBERTa} \cite{Qin2021ERICAIE}.  We fine-tune the pre-trained model on DocRED's human annotated train/dev/test splits for 200 epochs, using a batch size of 32 (see Appendix \ref{app:docred} for detailed experimental settings). Table \ref{tab:docred} reports performance across multiple data reduction settings (1\%, 10\%, and 100\%), using an overall F1-Micro score and an F1-Micro score computed by ignoring fact triples in the test set that overlap with fact triples in the training and development splits. We observe that \our outperforms all baselines and settings, offering evidence that \our produces better relationship representations from noisy data.


% DocRED Results
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l | c c | c c | c c } 
    \hline
    \rule{0pt}{3ex}
    \textbf{Size}               & \multicolumn{2}{c}{1\%}   & \multicolumn{2}{c}{10\%}  & \multicolumn{2}{c}{100\%} \\  \hline
    \rule{0pt}{3ex}
    \textbf{Metrics}            & F1     & IgF1      & F1    & IgF1      & F1    & IgF1  \\ \hline 
    \rule{-2pt}{3ex}
    CNN*                         & -      & -         & -     & -         & 42.3  & 40.3  \\ 
    BiLSTM*                      & -      & -         & -     & -         & 51.1  & 50.3  \\  \hline   
    \rule{-3pt}{3ex}
    HINBERT*                     & - & - & - & - & 55.6 & 53.7 \\
    CorefBERT*                   & 32.8 & 31.2 & 46.0 & 43.7 & 57.0 & 54.5 \\
    SpanBERT*                    & 32.2 & 30.4 & 46.4 & 44.5 & 57.3 & 55.0 \\
    ERNIE*                       & 26.7 & 25.5 & 46.7 & 44.2 & 56.6 & 54.2 \\
    MTB*                         & 29.0 & 27.6 & 46.1 & 44.1 & 56.9 & 54.3 \\
    CP*                          & 30.3 & 28.7 & 44.8 & 42.6 & 55.2 & 52.7 \\
    BERT                        & 19.9 & 18.8 & 45.2 & 43.1 & 56.6 & 54.4 \\
    RoBERTa                     & 29.6 & 27.9 & 47.6 & 45.7 & 58.2 & 55.9 \\
    ERICA\textsubscript{BERT}   & 22.9 & 21.7 & 48.5 & 46.4 & 57.4 & 55.2 \\
    ERICA\textsubscript{RoBERTa}& 30.0 & 28.2 & 50.1 & 48.1 & 59.1 & 56.9 \\ \hline
    \rule{-3pt}{3ex}
    \our                        & \textbf{33.2} & \textbf{31.2} & \textbf{50.3} & \textbf{48.3} & \textbf{59.4} & \textbf{57.1} \\ \hline
\end{tabular}} %end resize
\caption{F1-micro scores reported on the DocRED test set. IgF1 ignores performance on fact triples in the test set overlapping with triples in the train/dev sets. (* denotes performance as reported in \cite{Qin2021ERICAIE}, all other numbers are from our own implementations).}
\label{tab:docred}
\end{table}


% TACRED & SemEval Results
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l | c c c | c c c } 
    \hline
    \rule{0pt}{3ex}
    \textbf{Dataset}               & \multicolumn{3}{c}{TACRED}   & \multicolumn{3}{c}{SemEval} \\  \hline
    \rule{-3pt}{3ex}
    \textbf{Size}               & 1\%     & 10\%      & 100\%    & 1\%      & 10\%    & 100\%  \\ \hline 
    \rule{-3pt}{3ex}
    MTB*                            & 35.7 & 58.8 & 68.2 & 44.2 & 79.2 & 88.2 \\
    CP*                             & 37.1 & 60.6 & 68.1 & 40.3 & 80.0 & 88.5 \\ 
    BERT                            & 22.2 & 53.5 & 63.7 & 41.0 & 76.5 & 87.8 \\
    RoBERTa                         & 27.3 & 61.1 & 69.3 & 43.6 & 77.7 & 87.5 \\
    ERICA\textsubscript{BERT}       & 34.9 & 56.0 & 64.9 & 46.4 & 79.8 & 88.1 \\
    ERICA\textsubscript{RoBERTa}    & 41.1 & 61.7 & 69.5 & 50.3 & 80.9 & 88.4 \\ \hline
    \rule{-3pt}{3ex}
    \our                & \textbf{43.7} & \textbf{62.7} & \textbf{70.3} & \textbf{51.2} & \textbf{81.0} & \textbf{88.7}\\ \hline
\end{tabular}} %end resize
\caption{F1-micro scores reported from the TACRED and SemEval test sets (* denotes performance as reported in \cite{Qin2021ERICAIE}, all other numbers are from our own implementations).}
\label{tab:tacred_semeval}
\end{table}


\textbf{Sentence-level RE}: To assess our framework's ability to extract sentence-level relations, we report performance on TACRED \cite{zhang2017tacred} and SemEval-2010 Task 8 \cite{hendrickx-etal-2010-semeval}. We compare our model to MTB, CP, BERT, RoBERTa, ERICA\textsubscript{BERT}, and ERICA\textsubscript{RoBERTa} (see Appendix \ref{app:semeval_tacred} for detailed experimental settings). Table \ref{tab:tacred_semeval} reports F1 scores across multiple data reduction settings (1\%, 10\%, 100\%). We, again, observe an increase in performance in all settings using \our compared to the baselines. 


==> archive/_4_finecl_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% FGCL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Contrastive Pre-training}\label{sec:experiments}

\subsection{Overview}
This section introduces our pre-training method to learn high-quality entity and relation representations. We first construct informative representation for entities and relationships which we use to implement a three-part pre-training objective that features entity discrimination, relation discrimination, and masked language modeling. 

\subsection{Entity \& Relation Representation}\label{sec:entity_relation_repr}
We construct entity and relationship representations following ERICA~\cite{Qin2021ERICAIE}. For the document $d_i$, we use a pre-trained language model to encode $d_i$ and obtain the hidden states $\{\mathbf{h}_1, \mathbf{h}_2,\dots,\mathbf{h}_{|d_i|}\}$. Then, \textit{mean pooling} is applied to the consecutive tokens in entity $e_j$ to obtain entity representations. Assuming $n_{\mathrm{start}}$ and $n_{\mathrm{end}}$ are the start index and end index of entity $e_j$ in document $d_i$, the entity representation of $e_j$ is represented as:
\begin{equation}
    \mathbf{m}_{e_j} = \mathrm{MeanPool}(\mathbf{h}_{n_{\mathrm{start}}},\dots,\mathbf{h}_{n_{\mathrm{end}}}),
\end{equation}
To form a relation representation, we concatenate the representations of two entities $e_{j1}$ and $e_{j2}$: $\mathbf{r}_{j1j2} = [\mathbf{e}_{j1};\mathbf{e}_{j2}]$. 

\subsection{Entity Discrimination}
For entity discrimination, we use the same method described in ERICA. The goal of entity discrimination is inferring the tail entity in a document given a head entity and a relation~\cite{Qin2021ERICAIE}. The model distinguishes the ground-truth tail entity from other entities in the text. Given a sampled instance tuple $t^i_jk = (d_i, e_{ij}, r^i_{jk}, e_{ik})$, our model is trained to distinguish the tail entity $e_{ik}$ from other entities in the document $d_i$. Specifically, we concatenate the relation name of $r^i_{jk}$, the head entity $e_{ij}$ and a special token \texttt{[SEP]} in front of $d_i$ to get $d^*_i$. Then, we encode $d^*_i$ to get the entity representations using the method from Section~\ref{sec:entity_relation_repr}. The contrastive learning objective for entity discrimination is formulated as:
\begin{equation}
    \mathcal{L}_{\mathrm{ED}}=-\sum_{t_{j k}^{i} \in \mathcal{T}^\prime} \log \frac{\exp \left(\cos \left(\mathbf{e}_{i j}, \mathbf{e}_{i k}\right) / \tau\right)}{\sum_{l=1, l \neq j}^{\left|\mathcal{E}_{i}\right|} \exp \left(\cos \left(\mathbf{e}_{i j}, \mathbf{e}_{i l}\right) / \tau\right)},
\end{equation}
where $\mathrm{cos}(\cdot,\cdot)$ denotes the cosine similarity between two entity representations and $\tau$ is a temperature hyper-parameter.

\subsection{Relation Discrimination}
%\jingbo{will people be confused between RE and RD? Maybe spend one sentence to explain their relationship and why we are doing RD here.}
To effectively learn representation for downstream task relation extraction, we conduct a Relation Discrimination (RD) task during pre-training. RD aims to distinguish whether two relations are semantically similar~\cite{Qin2021ERICAIE}. Existing methods~\cite{Peng2020LearningFC, Qin2021ERICAIE} require large amounts of automatically labeled data from distant supervision which is noisy because not all sentences will adequately express a relationship.

In this case, the learning order can be introduced to make the model aware of the noise level of relation instances. To efficiently incorporate learning order into the training process, we propose fine-grained, noise-aware relation discrimination.

%\jingbo{I think the title, abstract, intro are all saying \our is proposed for RE}
In this new method, the noise level of all distantly supervised training instances controls the optimization process by re-weighting the contrastive objective. Intuitively, the model should learn more from high-quality, accurately labeled training instances than noisy, inaccurately labeled instances. Hence, we assign higher weights to earlier learned instances from the learning order denoising stage.

In practice, we sample a tuple pair of relation instance $t_A = (d_A, e_{A_1}, r_A, e_{A_2}, k_A)$ and $t_B = (d_B, e_{B_1}, r_B, e_{B_2}, k_B)$ from $\mathcal{T}^\prime$ and $r_A = r_B$, where $d$ is a document; $e$ is a entity in $d$; $r$ is the relationship between two entities and $k$ is the first learned order introduced in Section~\ref{sec:learning_order}. Using the method mentioned in Section~\ref{sec:entity_relation_repr}, we obtain the positive relation representations $\mathbf{r}_{t_A}$ and $\mathbf{r}_{t_B}$. To discriminate positive examples from negative ones, the fine-grained RD is defined as follows:
\begin{equation}
\begin{aligned}
\mathcal{L}_{\mathrm{RD}} &=-\sum_{t_{A}, t_{B} \in \mathcal{T}^\prime}f(k_A)\log \frac{\exp \left(\cos \left(\mathbf{r}_{t_{A}}, \mathbf{r}_{t_{B}}\right) / \tau\right)}{\mathcal{Z}}, \\
\mathcal{Z} &=\sum_{t_{C} \in \mathcal{T}^\prime /\left\{t_{A}\right\}}^{N} f(k_C)\exp \left(\cos \left(\mathbf{r}_{t_{A}}, \mathbf{r}_{t_{C}}\right) / \tau\right) \\
\end{aligned}
\end{equation}
Where $\mathrm{cos}(\cdot,\cdot)$ denotes the cosine similarity; $\tau$ is the temperature; $N$ is a hyper-parameter and $t_{C}$ is a negative instance ($r_A \neq r_C$) sampled from $\mathcal{T}^\prime$. Relation instances $t_A$ and $t_C$ are re-weighted by function $f$ which is defined as:
\begin{equation}
    f(k) = \alpha^{\frac{k_{\mathrm{max}}-k}{k_{\mathrm{max}}- k_{\mathrm{min}}}},
\end{equation}
where $\alpha$ ($\alpha > 1$) is a hyper-parameter that weighs the negative samples; $\mathrm{max}$ and $\mathrm{min}$ are maximum and minimum first-learned order, respectively. We increase the weight of negative $t_C$ if it is a high-quality training instance (i.e.,~$k$ is small). Because all positives and negatives are discriminated from instance $t_A$, we control the overall weight by the learning order $k_A$.

% \mathcal{L}_{\mathrm{RD}} &=\mathcal{L}_{\mathrm{RD}}^{\mathcal{T}_{s}^{+}, \mathcal{T}_{s}^{+}}+\mathcal{L}_{\mathrm{RD}}^{\mathcal{T}_{s}^{+}, \mathcal{T}_{c}^{+}}+\mathcal{L}_{\mathrm{RD}}^{\mathcal{T}_{c}^{+}, \mathcal{T}_{s}^{+}}+\mathcal{L}_{\mathrm{RD}}^{\mathcal{T}_{c}^{+}, \mathcal{T}_{c}^{+}}
% \end{aligned}

\subsection{Overall Objective}
We include the MLM task~\cite{Devlin2019BERTPO} to avoid catastrophic forgetting of language understanding~\cite{McCloskey1989CatastrophicII} and construct the following overall objective for \our:
\begin{equation}
\mathcal{L}_{FineCL} = \mathcal{L}_{ED} + \mathcal{L}_{RD} + \mathcal{L}_{MLM} 
\end{equation}

% 
% Pre-training
% 
\subsection{Pre-training Details}
To ensure a fair comparison and highlight the effectiveness of Fine-grained Contrastive Learning, we align our pre-training data and settings to those used by ERICA. The pre-training dataset provided by \cite{Qin2021ERICAIE} is constructed using distant supervision for RE by pairing documents from Wikipedia (English) with the Wikidata knowledge graph. This distantly labeled dataset creation method mirrors the method used to create the distantly labeled training set in DocRED \cite{docred} but differs in that it is much larger and more diverse. It contains 1M documents, 7.2M relation instances, and 1040 relation types compared to DocRED's 100k documents, 1.5M relation instances, and 96 relation types (not including \textit{no relation}). Additional checks are performed to ensure no fact triples overlap between the training data and the test sets of the various downstream RE tasks.



% 
% DocRED Results
% 
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l | c c | c c | c c } 
    \hline
    \rule{0pt}{3ex}
    \textbf{Size}               & \multicolumn{2}{c}{1\%}   & \multicolumn{2}{c}{10\%}  & \multicolumn{2}{c}{100\%} \\  \hline
    \rule{0pt}{3ex}
    \textbf{Metrics}            & F1     & IgF1      & F1    & IgF1      & F1    & IgF1  \\ \hline 
    \rule{-2pt}{3ex}
    CNN*                         & -      & -         & -     & -         & 42.3  & 40.3  \\ 
    BiLSTM*                      & -      & -         & -     & -         & 51.1  & 50.3  \\  \hline   
    \rule{-3pt}{3ex}
    HINBERT*                     & - & - & - & - & 55.6 & 53.7 \\
    CorefBERT*                   & 32.8 & 31.2 & 46.0 & 43.7 & 57.0 & 54.5 \\
    SpanBERT*                    & 32.2 & 30.4 & 46.4 & 44.5 & 57.3 & 55.0 \\
    ERNIE*                       & 26.7 & 25.5 & 46.7 & 44.2 & 56.6 & 54.2 \\
    MTB*                         & 29.0 & 27.6 & 46.1 & 44.1 & 56.9 & 54.3 \\
    CP*                          & \underline{30.3} & \underline{28.7} & 44.8 & 42.6 & 55.2 & 52.7 \\
    BERT                        & 19.9 & 18.8 & 45.2 & 43.1 & 56.6 & 54.4 \\
    RoBERTa                     & 29.6 & 27.9 & 47.6 & 45.7 & 58.2 & 55.9 \\
    ERICA\textsubscript{BERT}   & 22.9 & 21.7 & 48.5 & 46.4 & 57.4 & 55.2 \\
    ERICA\textsubscript{RoBERTa}& 30.0 & 28.2 & \underline{50.1} & \underline{48.1} & \underline{59.1} & \underline{56.9} \\
    WCL\textsubscript{RoBERTa}  & 22.3 & 20.8 & 49.4 & 47.5 & 58.5 & 56.2 \\ \hline 
    \rule{-3pt}{3ex}
    \our                        & \textbf{33.2} & \textbf{31.2} & \textbf{50.3} & \textbf{48.3} & \textbf{59.5} & \textbf{57.1} \\ \hline
\end{tabular}} %end resize
\caption{F1-micro scores reported on the DocRED test set. IgF1 ignores performance on fact triples in the test set overlapping with triples in the train/dev sets. (* denotes performance as reported in \cite{Qin2021ERICAIE}; all other numbers are from our implementations).}
\label{tab:docred}
\end{table}

\subsection{Supervised Adaptation}\label{subsec:experiments_relation_extraction}
The primary focus of our work is to improve relationship representations learned during pre-training and, in doing so, improve performance on downstream RE tasks. To illustrate the effectiveness of our pre-training method, we use cross-entropy loss, as described in equation \ref{eq:cross_entropy}, to fine-tune our pre-trained \our model on document-level and sentence-level RE tasks. The baselines are pre-trained and fine-tuned with identical data and settings for a fair comparison.

\textbf{Document-level RE}: To assess our framework's ability to extract document-level relations, we report performance on DocRED \cite{docred}. We compare our model to the following baselines: (1) CNN \cite{zeng-etal-2014-relation}, (2) BiLSTM \cite{lstm}, (3) BERT \cite{Devlin2019BERTPO}, (4) RoBERTa \cite{Liu2019RoBERTaAR}, (5) MTB \cite{BaldiniSoares2019MatchingTB}, (6) CP \cite{Peng2020LearningFC}, (7 \& 8) ERICA\textsubscript{BERT} \& ERICA\textsubscript{RoBERTa} \cite{Qin2021ERICAIE}, (9) WCL\textsubscript{RoBERTa} \cite{Peng2020LearningFC}.  We fine-tune the pre-trained models on DocRED's human-annotated train/dev/test splits (see Appendix \ref{app:docred} for detailed experimental settings). We implement WCL with identical settings from our other pre-training experiments and, for a fair comparison, we use RoBERTa instead of BERT as the base model for WCL, given the superior performance we observe from RoBERTa in all other experiments. Table \ref{tab:docred} reports performance across multiple data reduction settings (1\%, 10\%, and 100\%), using an overall F1-micro score and an F1-micro score computed by ignoring fact triples in the test set that overlap with fact triples in the training and development splits. We observe that \our outperforms all baselines in all experimental settings, offering evidence  that \our produces better relationship representations from noisy data.

Given that learning-order denoising weighs earlier learned instances over later learned instances, \our may be biased towards easier, or common relation classes. The increase in F1-micro performance could result from improved predictions on common relation classes at the expense of predictions on rare classes. To better understand the performance gains, we also report F1-macro and F1-macro weighted in Table \ref{tab:macro_docred}. The results show that \our outperforms the top baselines in both F1-macro metrics indicating that, on average, our method improves performance across all relation classes. However, the low F1-macro scores from all the models highlights an area for improvement---future pre-trained RE models should focus on improving performance on long-tail relation classes. 


% 
% Macro and Weighted Macro
% 
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l | c | c } 
    \hline
    \rule{0pt}{3ex}
    \textbf{Metric}                 & F1-macro     & F1-macro-weighted \\ \hline 
    \rule{-3pt}{3ex}
    BERT                            & 37.3              & 54.9 \\
    RoBERTa                         & 39.6              & 56.9 \\
    ERICA\textsubscript{BERT}       & 37.9              & 55.8 \\
    ERICA\textsubscript{RoBERTa}    & \underline{40.1 } & \underline{57.8} \\ 
    WCL\textsubscript{RoBERTA}      & 39.9              & 57.2 \\ \hline
    \rule{-3pt}{3ex}
    \our                            & \textbf{40.7 }     & \textbf{58.2} \\ \hline
\end{tabular}} %end resize
\caption{F1-macro and F1-macro-weighted scores reported from the DocRED test set.}
\label{tab:macro_docred}
\end{table}


% 
% TACRED & SemEval Results
% 
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l | c c c | c c c } 
    \hline
    \rule{0pt}{3ex}
    \textbf{Dataset}               & \multicolumn{3}{c}{TACRED}   & \multicolumn{3}{c}{SemEval} \\  \hline
    \rule{-3pt}{3ex}
    \textbf{Size}               & 1\%     & 10\%      & 100\%    & 1\%      & 10\%    & 100\%  \\ \hline 
    \rule{-3pt}{3ex}
    MTB*                            & 35.7 & 58.8 & 68.2 & 44.2 & 79.2 & 88.2 \\
    CP*                             & 37.1 & 60.6 & 68.1 & 40.3 & 80.0 & \underline{88.5} \\ 
    BERT                            & 22.2 & 53.5 & 63.7 & 41.0 & 76.5 & 87.8 \\
    RoBERTa                         & 27.3 & 61.1 & 69.3 & 43.6 & 77.7 & 87.5 \\
    ERICA\textsubscript{BERT}       & 34.9 & 56.0 & 64.9 & 46.4 & 79.8 & 88.1 \\
    ERICA\textsubscript{RoBERTa}    & \underline{41.1} & \underline{61.7} & 69.5 & \underline{50.3} & \underline{80.9} & 88.4 \\ 
    WCL\textsubscript{RoBERTA}      & 37.6 & 61.3 & \underline{69.7} & 47.0 & 80.0 & 88.3 \\ \hline
    \rule{-3pt}{3ex}
    \our                & \textbf{43.7} & \textbf{62.7} & \textbf{70.3} & \textbf{51.2} & \textbf{81.0} & \textbf{88.7}\\ \hline
\end{tabular}} %end resize
\caption{F1-micro scores reported from the TACRED and SemEval test sets (* denotes performance as reported in \cite{Qin2021ERICAIE}; all other numbers are from our implementations).}
\label{tab:tacred_semeval}
\end{table}


\textbf{Sentence-level RE}: To assess our framework's ability to extract sentence-level relations, we report performance on TACRED \cite{zhang2017tacred} and SemEval-2010 Task 8 \cite{hendrickx-etal-2010-semeval}. We compare our model to MTB, CP, BERT, RoBERTa, ERICA\textsubscript{BERT}, ERICA\textsubscript{RoBERTa}, and WCL\textsubscript{RoBERTa} (see Appendix \ref{app:semeval_tacred} for detailed experimental settings). Table \ref{tab:tacred_semeval} reports F1 scores across multiple data reduction settings (1\%, 10\%, 100\%). Again, we observe an increase in performance in all settings compared to the baselines.
